The DECam Local Volume Exploration Survey Data Release 2

We present the second public data release (DR2) from the DECam Local Volume Exploration survey (DELVE). DELVE DR2 combines new DECam observations with archival DECam data from the Dark Energy Survey, the DECam Legacy Survey, and other DECam community programs. DELVE DR2 consists of ~160,000 exposures that cover >21,000 deg^2 of the high Galactic latitude (|b| > 10 deg) sky in four broadband optical/near-infrared filters (g, r, i, z). DELVE DR2 provides point-source and automatic aperture photometry for ~2.5 billion astronomical sources with a median 5{\sigma} point-source depth of g=24.3, r=23.9, i=23.5, and z=22.8 mag. A region of ~17,000 deg^2 has been imaged in all four filters, providing four-band photometric measurements for ~618 million astronomical sources. DELVE DR2 covers more than four times the area of the previous DELVE data release and contains roughly five times as many astronomical objects. DELVE DR2 is publicly available via the NOIRLab Astro Data Lab science platform.

==> table_crossmatch.tex <==
\begin{deluxetable}{l l c}
    	\centering
	\tablewidth{0pt}
	\tabletypesize{\scriptsize}
	\tablecaption{DELVE DR2 crossmatch table descriptions. \label{tab:dr2_crossmatch}}
	\tablehead{
		\colhead{Column Name} & \colhead{Description} & \colhead{Columns}
	}
        \startdata
	DEC1 & Declination from DELVE DR2 (deg) & 1\\
	DEC2 & Declination from external catalog (deg) & 1\\
        DISTANCE & Angular separation between RA1,DEC1 and RA2,DEC2 (arcsec) & 1 \\
        ID1 & ID in DELVE DR2 (\var{quick\_object\_id}) & 1 \\
        ID2 & ID in external catalog & 1 \\
        RA1 & Right ascension from DELVE DR2 (deg) & 1 \\
        RA2 & Right ascension from external catalog (deg) & 1 \\
\enddata
\end{deluxetable}

